Continuous Jumping for Legged Robots on Stepping Stones via Trajectory Optimization and Model Predictive Control

Performing highly agile dynamic motions, such as jumping or running on uneven stepping stones has remained a challenging problem in legged robot locomotion. This paper presents a framework that combines trajectory optimization and model predictive control to perform robust and consecutive jumping on stepping stones. In our approach, we first utilize trajectory optimization based on full-nonlinear dynamics of the robot to generate periodic jumping trajectories for various jumping distances. A jumping controller based on a model predictive control is then designed for realizing smooth jumping transitions, enabling the robot to achieve continuous jumps on stepping stones. Thanks to the incorporation of MPC as a real-time feedback controller, the proposed framework is also validated to be robust to uneven platforms with unknown height perturbations and model uncertainty on the robot dynamics.

==> Sections/AdaptiveSupportPolygon.tex <==
%!TEX root = ../Main.tex



% This is no longer a full section... make into a subsection in the Control part





\section{Predictive Support Polygon}
\label{sec:ASP}
\iffalse
\subsection{Nomenclature}

\subsubsection{Leg state Boolean variables}
\begin{itemize}
	\item $\legState \in \BMat{0 = swing, 1 = contact}$ : actual contact state of the foot
	\item $\legStateScheduled \in \BMat{0 = swing, 1 = contact}$ : scheduled contact state of the foot
	\item $\legStateNotScheduled \in \BMat{0 = contact, 1 = swing}$ : negation of the scheduled contact state of the foot
	\item $\legStateEstimated \in \BMat{0 = swing, 1 = contact}$ : estimated contact state of the foot
\end{itemize}

\subsubsection{Contact state subscripts}
\begin{itemize}
	\item $\contactState := \{\legState=1\}$ : denotes that the variable pertains to the actual contact state
	\item $\swingState := \{\legState=0\}$ : denotes that the variable pertains to the actual swing state
	\item $\contactStateScheduled := \{\legStateScheduled=1\}$ : denotes that the variable pertains to the scheduled contact state
	\item $\swingStateScheduled := \{\legStateScheduled=0\}$ : denotes that the variable pertains to the scheduled swing state
\end{itemize}

\subsubsection{Contact Model Parameters}
\begin{itemize}
	\item $\phi$ : phase variable for the overall gait cycle
	\item $\phi_{\contactState}$ : phase variable for the contact subphase
	\item $\phi_{\swingState}$ : phase variable for the swing subphase
	\item $p_{z}$ : measured foot height from kinematics and encoders
	\item $f_{z}$ : measured vertical force from the Inverse Dynamics force estimator
\end{itemize}

\subsubsection{Probabilistic Model Parameters}
\begin{itemize}
	\item $\mu_{z_{g}}$ : average expected ground height at the step location
	\item $\sigma_{z_{g}}^{2}$ : variance of the expected ground height, a loose measure of ground roughness 
	\item $\mu_{f_{c}}$ : average force that we expect to see when initiating contact
	\item $\sigma_{f_{c}}^{2}$ : variance for force at contact that comes from inconsistencies in the Inverse Dynamics model and sensor noise
\end{itemize}

\subsubsection{Probabilistic Model Random Variables}
\begin{itemize}
	\item $\Phi_{\contactState|\swingStateScheduled} \sim$ : the model for the phase at which contact occurs given that you are currently scheduled to be in swing
	\item $\Phi_{\swingState|\contactStateScheduled} \sim$ : the model for the phase at which you are not in contact occurs given that you are currently scheduled to be in contact
	\item $Z_g \sim \mathcal{N}(\mu_{z_{g}},\,\sigma_{z_{g}}^{2})$ : the model for ground height is drawn from a Normal Gaussian distribution
	\item $F_c \sim \mathcal{N}(\mu_{f_{c}},\,\sigma_{f_{c}}^{2})$ : the model for force at which contact occurs is drawn from a Normal Gaussian distribution
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%							Contact Probability Functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Adaptive Phase Gain}
We will first define a phase-based adaptive gain that gives a weighting for each foot's contribution to the support polygon. The goal is to design an informed nonlinear phase dependent gain by exploiting the robot's knowledge of which feet will be the next to lift off or touch down and when these state changes are scheduled to occur.

Phase gain contact
\begin{equation}
K_{\contactStateScheduled} = \frac{1}{2}\bMat{erf\pMat{\frac{\phi}{\sigma_{c_0}\sqrt{2}}} + erf\pMat{\frac{1-\phi}{\sigma_{c_1}\sqrt{2}}}}
\end{equation}
Phase gain swing
\begin{equation}
K_{\swingStateScheduled} = \frac{1}{2}\bMat{2+erf\pMat{\frac{-\phi}{\sigma_{\bar{c}_0}\sqrt{2}}} + erf\pMat{\frac{\phi-1}{\sigma_{\bar{c}_1}\sqrt{2}}}}
\end{equation}

\begin{figure}
	\center
	\includegraphics[width=0.92 \columnwidth]{Figures/K_contact.pdf}
	\caption{{\bfseries Contact Phase Gain.} .}
	\label{fig:K_swing}
\end{figure}


\begin{figure}
	\center
	\includegraphics[width=0.92 \columnwidth]{Figures/K_swing.pdf}
	\caption{{\bfseries Swing Phase Gain.} .}
	\label{fig:K_swing}
\end{figure}

\begin{equation}
\phaseGain = \legStateScheduled K_{\contactStateScheduled} + \legStateNotScheduled K_{\swingStateScheduled}
\end{equation}
where the boolean variable signifying scheduled contact state is defined as $\legStateScheduled \in \BMat{0 = swing,1 = contact}$. Roughly, this will tell the robot that the closer you are to the middle of your contact phase, the more you can trust that the leg can be used for balance, while the closer you are to the middle of the swing phase, the less you can trust that a leg can be used for balance. 


\subsection{Virtual Phase-Weighted points}
Using the phase-based weightings, we can define a set of virtual points for each leg. These virtual points act as a method to continuously weight the predicted relative availability of each leg to be used in stance when compared to its adjacent legs. These virtual points slide between the 2D ground projection line between the foot and the corresponding adjacent foot during the gait cycle. The two virtual points for leg $i \in \{FR, FL, BR, BL\}$ are defined as
\begin{equation}
\bm{\xi}_{i}\adjLegM = \phaseGain_{i}p_{i} + (1-\phaseGain_{i})p_{i\adjLegM}
\end{equation}
\begin{equation}
\bm{\xi}_{i}\adjLegP = \phaseGain_{i}p_{i} + (1-\phaseGain_{i})p_{i\adjLegP}
\end{equation}
\begin{equation}
\bMat{\bm{\xi}_{i}\adjLegM\\\bm{\xi}_{i}\adjLegP} = \phaseGain_{i}\bm{p}_{i}\bMat{1 \\ 1} + (1-\phaseGain_{i})\bMat{\bm{p}_{i\adjLegM}\\\bm{p}_{i\adjLegP}}
\end{equation}
\begin{equation}
\bMat{\bm{\xi}_{i}\adjLegM\\\bm{\xi}_{i}\adjLegP} = \bMat{\bm{p}_{i} & \bm{p}_{i\adjLegM} \\ \bm{p}_{i} &\bm{p}_{i\adjLegP}}\bMat{\phaseGain_{i}\\1-\phaseGain_{i}}
\end{equation}
where the superscript signifies that the quantity references the adjacent leg ordered backwards, $-$, or forwards, $+$, when considering iterating counterclockwise from above over the legs. As an example, we consider the virtual point defined by, $\bm{\xi}_{FL}\adjLegM = \phaseGain_{FL}\bm{p}_{FL} + (1-\phaseGain_{FL})\bm{p}_{FR}$. This virtual point would be located on the line between the front left foot position, $\bm{p}_{FL}$, and the front right foot position, $\bm{p}_{FR}$, at a distance proportional to $\Phi_{FL}$ away from the front left foot that it is associated with. Therefore, in the middle of the contact phase, $\bm{\xi}_{i}\adjLegM$, will be at its closest point to its associated foot position, $p_{i}$, and in the middle of the swing phase it will be closest to the adjacent foot position, $\bm{p}_{i\adjLegM}$.

With the current foot position, we can now describe the predictive support polygon vertex for leg $i$ to be
\begin{equation}
\bm{\xi}_i = \frac{\phaseGain_i\bm{p}_{i}+\sum\limits_{j \in \{-,+\}}\phaseGain_{f_{i}}\bm{\xi}^{j}_{i}}{\sum\limits_{i \in \{-,+\}}\phaseGain_{f_{i}}}
\end{equation}
\begin{equation}
\bm{\xi}_i = \frac{\phaseGain_{i}\bm{p}_{i} + \phaseGain_{i\adjLegM}\bm{\xi}_i\adjLegM+\phaseGain_{i\adjLegP}\bm{\xi}_i\adjLegP}{\phaseGain_{i}+\phaseGain_{i\adjLegM}+\phaseGain_{i\adjLegP}}
\end{equation}
where $f_{i}$ is the $i^{th}$ relative foot to foot $f$.
Desired CoM position
\begin{equation}
\hat{\bm{p}}_{CoM,d} = \frac{\sum\limits_{i = 1}^{N}\bm{\xi}_{i}}{N}
\end{equation}


\begin{figure}
	\center
	\includegraphics[width=0.65 \columnwidth]{Figures/support_polygon_point_definitions_no_lines.pdf}
	\caption{{\bfseries Point Definitions.} The definitions for the various points used to define the predictive support polygon. Shown during a trotting gait with zero velocity command.}
	\label{fig:PointDefinitions}
\end{figure}



Figure \ref{fig:PointDefinitions} shows the interaction of the virtual points to create the predictive support polygon during a trotting gait. The dashed line shows the actual support polygon between the two stance feet. Since the we model contacts using point feet, there is only a line of support in which the robot can be statically stable. However, by using the virtual support polygon, the robot can afford for the CoM to be located outside of the actual support polygon, knowing that it will soon be in the new support polygon when the contact mode switches.







\section{Dynamic Gaits}

Figure XXXXXXXXXXXX shows that during pacing, the robot is never 

==> Sections/ControlArchitecture.tex <==
%!TEX root = ../Main.tex

\begin{figure*}[t!]
	\center
	\includegraphics[width=2 \columnwidth]{Figures/BD-crop.pdf}
	\caption{{\bfseries System Architecture Block Diagram.} The user sends velocity and turning commands as well as general tunable parameters to the main computer. The main Cheetah control computer is composed of three main parts: higher-level planning (green), leg and body control (red), and state estimation (blue). The force and position commands are sent to the microcontrollers for each leg that relay the motor command to the robot.}
	\label{fig:BD}
\end{figure*}

\section{Control Architecture}
\label{sec:CA}

The overall architecture of the system is depicted in the block diagram in Figure \ref{fig:BD}. Each block is designed to be modular so it can be easily substituted without any modification to the other parts of the system. The operator provides high-level commands by giving a desired translational velocity, $\dot{\bm{p}}_d$, and turning rate, $\dot{\psi}_d$. These commands are used to plan a smooth and controllable CoM reference trajectory that is relayed to the body and leg controllers. Various controllers and planners use the user-input commands and the estimated robot state to generate force commands if the leg is in stance or position commands if the leg is in swing. The following sections describe the implementation of the major components of the system on the MIT Cheetah~3.% robot platform.


%The robot uses an IMU to get angular rates in the body frame, ${}^\mathcal{B}\bm{\omega}$, and the acceleration of the body, $\bm{\ddot{p}}$. Encoders provide the joint angles, $\bm{q}$, for all of the leg joints.

%Various controllers can be used to plan out ground reaction forces to track the desired CoM trajectories. 


\subsection{Gait Planning}\label{sec:GP}

The Cheetah's gait is defined by an event-based finite state machine that uses a leg-independent phase variable to schedule nominal contact and swing phases. This allows for flexible gait definitions and fluid transitions between them. Trotting, bounding, and pacing gaits are presented in this paper, but the framework allows implementation of any gait definition with ease. The gaits were designed to mimic natural animal gaits by controlling the independent phases of each leg. This nominal gait plan is modified during unexpected contact events on the legs. Since the robot does not use any external environment sensors, a contact detection algorithm probabilistically fuses encoder measurements, estimated force, and expected gait phase to estimate the likelihood that each leg is in contact with an object \cite{Bledt18}. Scheduled contacts are defined by independent boolean variables $\legStateScheduled \in \BMat{0 = swing,1 = contact}$, while estimated contacts are given by $\legStateEstimated \in \BMat{0 = swing,1 = contact}$.  With this information, the robot can differentiate between normal operation, unexpected early contacts, and late missed contacts to adjust its control actions appropriately \cite{Bledt18}.


\input{Sections/Kinematics.tex}



\input{Sections/ForceControlQP.tex}


\subsection{Force Control - Model Predictive Control}\label{sec:MPC}
As an alternative to the Balance Controller, the ground force control block can be replaced with a model-predictive controller (MPC) that reasons about trajectory outcomes over a longer temporal horizon.  A model-predictive force-planning approach can be formulated to plan ground reaction forces $\bm{u}$ to minimize a cost function
\begin{align}
J = \sum_{i = 0}^k (\bm{x}_i - \bm{x}_i^{\text{ref}})^\top \bm{Q}_i (\bm{x}_i - \bm{x}_i^{\text{ref}}) + \bm{u}_i^\top \bm{R}_i\bm{u}_i
\end{align}
where $\bm{Q}_i$ and $\bm{R}_i$ are positive semidefinite matrices of weights, $\bm{x}_i \in \mathbb{R}^{12}$ is the robot's state at timestep $i$, consisting of position, velocity, orientation, and angular velocity, $\bm{x}_i^\text{ref}$ is the desired state of the robot,  and $k$ is the horizon length. Solving this MPC is challenging, as orientation dynamics have nonlinear coupled effects. In recent work \cite{DiCarlo18} approximate dynamics are enforced with linear equality constraints based on a time-varying approximation that enables formulating the MPC problem as a quadratic program.  The resulting controller is able to anticipate and plan around periods of flight and underactuation. Optimal forces are updated at 30 Hz and are sent directly to the leg controllers \cite{DiCarlo18}.

\subsection{Swing Leg Control}
% flat ground with zero height
Each of the footstep locations are calculated from the corresponding hip location using a linear combination of the Raibert heuristic \cite{Raibert86} and a velocity-based feedback term from the capture point formulation \cite{Pratt06}. Since the robot does not have external environment sensors{}, the footstep locations are projected onto an assumed ground plane. Therefore, the step location on the 2D ground plane for foot $i$ is calculated from the hip of the robot by the following
\begin{align}
	\label{eq:foot_pos}
	\bm{p}_{step,i} & = \pos_{h,i} + \underbrace{\frac{T_{\contactStateScheduled}}{2} \dot{\pos}_{c,d}}_{\text{Raibert Heuristic}} + \underbrace{\sqrt{\frac{z_0}{\|\bm{g}\|}}(\dot{\pos}_c - \dot{\pos}_{c,d})}_{\text{Capture Point}}
\end{align}
where $T_{\contactStateScheduled}$ is the nominal scheduled contact phase (stance) time, $z_0$ is the nominal height of locomotion, and $\pos_{h,i}$ provides the position of the corresponding hip $i$.


A PD controller with a feedforward term is used to compute joint torques for tracking the Cartesian swing trajectory for each foot.  The feedforward force is computed on the onboard embedded PC at 1 kHz using the leg dynamics
\begin{align}
\bm{\tau}_{\text{ff},i} = \bm{J}_i^\top \bm{\Lambda}_i({}^\mathfrak{B} \bm{a}_{i,\text{ref}} - \dot{\bm{J}}_i \dot{\bm{q}_i}) + \bm{C}_i \dot{\bm{q}}_i + \bm{G}_i
\end{align}
where $\bm{J}_i$ is the foot Jacobian, $\bm{\Lambda}_i$ is the operational space inertia matrix, ${}^\mathfrak{B} \bm{a}_{i,\text{ref}}$ is the reference acceleration for the swing trajectory, $\bm{q}_i$ is a vector of joint configurations, $\bm{C}_i$ is the Coriolis matrix, and $\bm{G}_i$ is the torque due to gravity.  The full controller for tracking swing trajectories is
\begin{align}
\bm{\tau}_i = \bm{J}_i^\top[\bm{K}_p({}^\mathfrak{B} \bm{p}_{i,\text{ref}} - {}^\mathfrak{B} \bm{p}_i) + \bm{K}_d({}^\mathfrak{B}\bm{v}_{i,\text{ref}} - {}^\mathfrak{B} \bm{v}_i)] + \bm{\tau}_{\text{ff},i}
\end{align}
where $\bm{K}_p$ and $\bm{K}_d$ are diagonal matrices of proportional and derivative gains.  The Cartesian PD controller runs on the leg controllers at 4.5 kHz.


To ensure the swing-leg PD controller remains stable, the gains are scaled with the apparent mass of the leg to maintain approximately the same natural frequency
\begin{align}
K_{p,j} = \omega_\text{des} \Lambda_{jj}(\bm{q})
\end{align}
where $K_{p,j}$ is the $j$-th diagonal entry in $\bm{K}_p$, $\omega_\text{des}$ is the desired natural frequency, and $\Lambda_{jj}$ is the $j$-th diagonal entry in the operational space inertia matrix.


\subsection{Virtual Predictive Support Polygon}
In order to take advantage of the hybrid nature of legged locomotion, a virtual support polygon is defined to provide a desired CoM location that generalizes across all gaits. By anticipating contact mode switches, the virtual support polygon biases away from legs nearing the end of their contact phase and towards legs about to touchdown. This strategy enables the robot to maintain its forward momentum during the gait while using selected footstep locations to create a smooth reference trajectory that is automatically adapted to the footholds online.

We define a phase-based approach that assigns each foot's contribution to the predictive support polygon, including feet in swing. 
The goal is to design an informed nonlinear phase-dependent weighting strategy by exploiting the robot's knowledge of which feet will be the next to lift off or touch down and when these state changes are scheduled to occur. 
Weighting factors are generated based on the contact and swing phases
%=======
%A phase-based weighting factor assigns weight to each foot's contribution to the virtual support polygon. The goal is to design an informed phase-dependent weighting strategy by exploiting the robot's knowledge of which feet will be the next to lift off or touch down and when these state changes are scheduled to occur. The weighting factors are composed of a curve for each of the contact and swing phases
%>>>>>>> c7308012ccbc28376b0b36353d5ca58e0a098217
\begin{equation}
K_{\contactStateScheduled} = \frac{1}{2}\bMat{ {\rm erf}\!\pMat{\frac{\phi}{\sigma_{c_0}\sqrt{2}}} + {\rm erf}\!\pMat{\frac{1-\phi}{\sigma_{c_1}\sqrt{2}}}}
\end{equation}
\begin{equation}
K_{\swingStateScheduled} = \frac{1}{2}\bMat{2+{\rm erf}\!\pMat{\frac{-\phi}{\sigma_{\bar{c}_0}\sqrt{2}}} + {\rm erf}\!\pMat{\frac{\phi-1}{\sigma_{\bar{c}_1}\sqrt{2}}}}
\end{equation}
\begin{equation}
\phaseGain = \legStateScheduled K_{\contactStateScheduled} + \legStateNotScheduled K_{\swingStateScheduled}
\end{equation}
where $K_{\contactStateScheduled}$ and $K_{\swingStateScheduled}$ correspond to the adaptive weighting factor during the scheduled contact and swing phase respectively. The quantity $\phaseGain$ represents the total weighting factor for the foot.  Roughly, this notifies the robot that the closer the leg is to the middle of its contact phase, the more confidently the robot can rely on that the leg as a support point, while the closer it is to the middle of the swing phase, the less the leg can be used for balance in the near future. 

%<<<<<<< HEAD
Using the phase-based weighting factors, a set of virtual points is defined for each leg. These virtual points lend a method to continuously weight the predicted relative availability of each leg as compared to its adjacent legs. These virtual points slide between the 2D ground projection line between the foot and the corresponding adjacent foot during the gait cycle. Each leg, $i \in \{FR, FL, BR, BL\}$, has two virtual points given by
%
%=======
%Using the phase-based weighting factors, a set of virtual points for each leg acts as a method to continuously weight the predicted relative availability of each leg as compared to its adjacent legs. These virtual points slide between the 2D ground projection line between a foot and its corresponding adjacent foot during the gait cycle. Each leg, $i \in \{FR, FL, BR, BL\}$, has two virtual points given by
%>>>>>>> c7308012ccbc28376b0b36353d5ca58e0a098217
\begin{equation}
\bMat{\bm{\xi}_{i}\adjLegM\\\bm{\xi}_{i}\adjLegP} = \bMat{\bm{p}_{i} & \bm{p}_{i\adjLegM} \\ \bm{p}_{i} &\bm{p}_{i\adjLegP}}\bMat{\phaseGain_{i}\\1-\phaseGain_{i}}
\label{eq:VPs}
\end{equation}
where the superscript signifies a reference to the adjacent leg clockwise, $-$, or counterclockwise, $+$. With the current foot position, we can now describe the predictive support polygon vertex for leg $i$ to be
\begin{equation}
\bm{\xi}_i = \frac{\phaseGain_{i}\bm{p}_{i} + \phaseGain_{i\adjLegM}\bm{\xi}_i\adjLegM+\phaseGain_{i\adjLegP}\bm{\xi}_i\adjLegP}{\phaseGain_{i}+\phaseGain_{i\adjLegM}+\phaseGain_{i\adjLegP}}
\label{eq:VP}
\end{equation}
The desired CoM position is then given as the average of these weighted virtual support polygon vertices
\begin{equation}
\hat{\bm{p}}_{CoM,d} = \frac{1}{N} \sum\limits_{i = 1}^{N}\bm{\xi}_{i} 
\end{equation}
Figure \ref{fig:PointDefinitions} shows an example evolution of this virtual predictive support polygon during trotting, but the method extends to all gaits. The virtual points defined in \eqref{eq:VPs} and \eqref{eq:VP} are labeled for the front right foot. In the sequence, the CoM moves from the support line in the middle of stance, towards the future support polygon as it expects the swing feet to touchdown and provide support.

%%%%%%%% These were from the old version of my paper... may not be as important in the overall implementation:

%This paper presents a novel method to exploit the dynamic nature of legged locomotion by anticipating contact mode switches within a short time horizon. A virtual support area is defined from the foot locations weighted by their expectation 

%trust that each leg will be useful for repositioning the CoM in the future

% By anticipating foot touchdown and liftoff events, the robot can embrace 

% This results in allowing the robot's center of mass (CoM) to fluidly follow the foot contact points rather than force undesirable foot locations in an attempt to follow a rigidly defined CoM trajectory. With this, the robot is able to steadily move using gaits that are rarely instantaneously statically stable.

% Rather than attempting to instantaneously track an absolute CoM position in the world, the robot uses the footstep locations to maintain balance, while positioning the CoM favorably relative to the dynamic foot locations.

\begin{figure}[t!]
	\center
	\includegraphics[width=0.33 \columnwidth]{Figures/SP_t1-crop.pdf}\quad\quad\quad
	\includegraphics[width=0.36 \columnwidth]{Figures/SP_t2-crop.pdf}
    
    \vspace{0.5cm}
	
	\includegraphics[width=0.36 \columnwidth]{Figures/SP_t3-crop.pdf}\quad\quad\quad
	\includegraphics[width=0.36 \columnwidth]{Figures/SP_t4-crop.pdf}
	\caption{{\bfseries Predictive Support Polygon.} As the robot trots with velocity to the right, the predictive support polygon (solid black) anticipates leg touchdown and guides the CoM away from the instantaneous physical support line (dashed black) towards the future support as contact modes switch. The vertices of the predictive support polygon are given by $\bm{\xi}_i$.}
	\label{fig:PointDefinitions}
\end{figure}

\input{Sections/LeastSquaresPitchPlane.tex}


\input{Sections/StateEstimation}



==> Sections/Design.tex <==
%!TEX root = ../Main.tex

\section{Design}
\label{sec:Design}

\begin{table}[t!]
	\centering
	\caption{Physical Robot Parameters}
	\label{tab:PRP}
	\begin{tabular}{cccc}
		\hline
		Parameter & Symbol & Value & Units\\
		\hline
		Mass & $m$    & 45 & $\unit{kg}$  \\[.5ex]
		Body Inertia  & $I_{xx}$  & 0.35 & $\unit{kg}\cdot \unit{m}^2$ \\[.5ex]
		 & $I_{yy}$ & 2.1  & $\unit{kg}\cdot \unit{m}^2$ \\[.5ex]
		 & $I_{zz}$ & 2.1  & $\unit{kg}\cdot \unit{m} ^2$ \\[.5ex]
		Body Length & $l_{body}$ & 0.600 & $\unit{m}$ \\[.5ex]
		Body Width & $w_{body}$ & 0.256 & $\unit{m}$ \\[.5ex]
		Body Height & $h_{body}$ & 0.200 & $\unit{m}$ \\[.5ex]
		Leg Link Lengths & $l_{1}, l_{2}$ & 0.34 & $\unit{m}$ \\[.5ex]
		\hline 
		\label{tab:robot}
	\end{tabular}
\end{table}



\subsection{Overview}
	The hardware design of Cheetah 3 builds on the actuation paradigm of the MIT Cheetah 1 and 2 robots \cite{Wensing17b}.  By using high torque density electric motors with backdriveable single-stage planetary gear reductions, and low-inertia legs, the Cheetah 3 robot can control ground reaction forces through proprioception, without the use of any force sensors, torque sensors, or series compliance at the joints or feet.  The Cheetah 2 robot was designed primarily for fast locomotion in the sagittal plane, and used high performance actuators at the hip and knee joints, but not for abduction/adduction (ab/ad).  Cheetah 3 has nearly identical actuators on all three degrees of freedom on each leg, enabling fully 3D control of ground reaction forces.  
	
	The Cheetah 3 legs feature a greatly expanded range of motion compared to Cheetah 2. The new ab/ad actuators have a range of motion of more than $\pm$45${}^{\circ}$, while new hip and knee designs allow the robot operate identically forwards, backwards, and flipped upside-down, and potentially use its legs for simple manipulation tasks as well as locomotion.
	
	The robot is powered by 450 Watt-hours of on-board Lithium Polymer batteries providing approximately 2 hours of run time,  although the robot has  internal space for twice the battery capacity, should longer run times be necessary.  
	
	
\subsection{Leg Design and Actuation}

\begin{figure}
	\center
	\includegraphics[width=1.0 \columnwidth]{Figures/LegDiagram-crop.pdf}
	\caption{{\bfseries Cheetah 3 Leg Design.} One leg showing the 3 actuators, with a cutaway view of the knee actuator.}
	\label{fig:LegDiagram}
\end{figure}
	
	The proprioceptive actuation strategy used on Cheetah 3 results in exceptional force bandwidth, force capability, and speed, at the cost of force accuracy compared to systems with closed-loop force control.  The static torque error of Cheetah 3's actuators is roughly $\pm$10\% primarily due to gear friction.  By comparison, the series elastic actuators used in ANYmal, which measure the deflection of a series spring to control output torque, have far greater torque accuracy, but much lower peak torque, speed, and torque bandwidth, especially at high torques \cite{7758092}.  However, we believe high force accuracy is not a requirement for dynamic legged locomotion, and our experiments have supported this claim.
	
	Each of Cheetah 3's actuators consists of a custom high torque density electric motor coupled to a single-stage 7.67:1 planetary gear reduction.  The slightly higher gear ratio compared to Cheetah 2 (5.8:1) was chosen to improve the load-carrying ability and low-speed efficiency of the robot.  The legs are serially actuated, but to keep leg inertia low, the hip and knee actuators are co-axially located at the hip of each leg as shown in Figure \ref{fig:LegDiagram}. 

	The lower link is driven by a roller chain which passes through the upper link, providing an additional 1.15x gear reduction.  By using a chain rather than a linkage, the lower link can rotate 330${}^{\circ}$, letting the robot arbitrarily change the orientation of its knees to point forwards or backwards. While the roller chain does introduce slight torque and speed ripple at the link, and adds some compliance between the knee actuator and the lower link, in practice these effects have not caused high-level performance to suffer.  

	The hip joint can rotate continuously, limited only by the length of the wires to the knee actuator, allowing the robot to potentially operate upside-down, climb up tall obstacles, or use its feet for manipulation above its body.  Two ab/ad actuators are located between each pair of legs, and are coupled to the legs by linkages.  See Figure \ref{fig:LegDiagram} for a cutaway view of leg actuation.  The leg links are machined aluminum, and in total have a mass of 2.7 kg for all four legs, or only 6\% of the mass of the robot.  The end of each leg has a cover made from 10mm thick 60A urethane rubber, providing cushioning and traction regardless of the contact angle between the leg and the ground.  Cheetah 3's actuation capabilities are summarized in Table \ref{tab:motor}.
	
		\begin{table}[t!]
	\centering
	\caption{Actuator Parameters}
	\begin{tabular}{cccc}
		\hline
		Parameter & Value & Units\\
		\hline
		Gear Ratio &   7.67   &   \\[.5ex]
		Max Torque   &  230 & $\unit{Nm}$  \\[.5ex]
		Max Joint Speed    & 21  & $\unit{Rad}/\unit{s}$  \\[.5ex]
		\hline 
		\label{tab:motor}
	\end{tabular}
\end{table}


	Cheetah 3's actuation system was designed to give the robot performance headroom for tasks including high speed locomotion, jumping, carrying loads, and recovering from extreme disturbances. As a simple performance metric, with the leg minimally extended, the robot is capable of producing a purely vertical ground reaction force of over 700 N, about 1.6 times the weight of the robot, \textit{per leg}.  And at 70\% extension, a  typical configuration during operation, vertical force capability exceeds 1000 N per leg.  By contrast, other quadruped robots for which data are available have far lower force-to-bodyweight capabilities: At minimal leg extension, ANYmal can produce around 0.54 bodyweights per leg \cite{7758092}, and HyQ2Max 0.84 bodyweights \cite{7587429}.  
	



\subsection{Computing and Low-Level Control Architecture}


	Cheetah 3 has a tiered computing architecture which enables low-level leg and motor control to be run at higher loop frequencies than locomotion control, and allows easy expansion of computing resources as needed for future sensing, planning, and navitgation tasks.  Locomotion control and state estimation are handled by the locomotion computer: an embedded PC with a 2nd Gen Core i7 laptop CPU, running Ubuntu Linux (kernel 4.1.33) with the CONFIG\textunderscore PREEMPT\textunderscore RT patch.  The locomotion computer receives user commands and logs data using Lightweight Communication and Marshalling (LCM) \cite{Olson10}.  LCM will allow additional computers for vision, planning, and other tasks to easily communicate with the locomotion computer in the future.  Leg-level control is performed by an ARM Cortex-A8-based processor.  The leg controller communicates with the locomotion computer at 1~kHz over EtherCAT, and performs leg-level control tasks like cartesian impedance control or joint PD control at 4.5~kHz.  The higher sample frequency at the leg level allows for high-rate joint velocity filtering as well as higher bandwidth tracking during swing phase and other position-controlled actions.  Finally, each leg controller sends torque commands and receives joint encoder measurements from the brushless motor drives for the three motors in each leg, which perform the current control on the motors at 20 kHz sample rate with 400 Hz closed-loop bandwidth.





==> Sections/FootstepPlacement.tex <==
%!TEX root = ../Main.tex


\section{Footstep Placement Controller}
\label{sec:FPC}


Each of the footstep locations are calculated using a linear combination of the Raibert heuristic for forward walking with the inverted pendulum dynamics \cite{Raibert86} and a velocity-based feedback term from the capture point formulation to correct for deviations from the desired trajectory \cite{Pratt06}. Since the robot does not have external environment sensors, the footstep locations are projected onto an assumed flat ground with zero height. Therefore, the step location on the 2D ground plane for foot $i$ is calculated from the CoM of the robot by the following
\begin{align}
	\label{eq:foot_pos}
	\bm{p}_{step,i} & = \pos_{h,i} + \underbrace{\frac{T_{\contactStateScheduled}}{2} \dot{\pos}_{c,d}}_{\text{Raibert Heuristic}} + \underbrace{\sqrt{\frac{z_0}{\|\bm{g}\|}}(\dot{\pos}_c - \dot{\pos}_{c,d})}_{\text{Capture Point}}
\end{align}

These



A PD controller is used to track a Cartesian position based swing trajectory for each foot. The swing foot trajectory is generated using the foot takeoff position and the desired footstep location defined in \ref{eq:foot_pos}. A set of B\'ezier polynomials are used to create smooth footstep trajectories between the takeoff and touchdown locations and are constantly updated to reflect any changes in the robot's state during swing.



==> Sections/ForceControlQP.tex <==
%!TEX root = ../Main.tex

\subsection{Force Control - Balance Controller}\label{sec:QP}
One of the Cheetah 3 support leg control modes is a Balance Controller, an implementation (with slight modification) of the controller described in \cite{Focchi17}. The Balance Controller enforces PD control on the center of mass and body orientation, while also ensuring that foot forces satisfy friction constraints. The PD control law is given by 
\begin{align}
\label{eq:pd_dynamics}
\left[\begin{array}{c}  \ddot{\pos}_{c,d} \\  \dot \bom_{b,d} \end{array} \right] = \left[\begin{array}{c}  \bm{K}_{p,p}(\pos_{c,d}-\pos_{c}) + \bm{K}_{d,p} (\dot{\pos}_{c,d}-\dot{\pos}_{c}) \\  \hspace{-0.1cm} \bm{K}_{p,\omega} \log(\bm{R}_d \bm{R}^T) +  \bm{K}_{d,\omega}(\bom_{b,d} - \bom)\end{array} \right]
\end{align}
The desired angular acceleration reflects PD control on $SO(3)$ wherein the desired and actual body orientations are described using rotation matrices $\bm{R}_d$ and $\bm{R}$, respectively, and the orientation error is obtained using the exponential map representation of rotations    \cite{Bullo95,MurrayLiSastry94}.


The goal of the Balance Controller is to resolve an optimal distribution of leg forces $\bm{F}$ that drive the approximate COM dynamics to the corresponding desired dynamics given by
\begin{align}
\bm{b}_d = \left[\begin{array}{c} m (\ddot{\pos}_{c,d} +\bm{g}) \\ \bm{I}_G \,\dot \bom_{b,d} \end{array} \right].
\end{align}
Since the model \eqref{eq:linear_model} is linear, the controller can naturally be expressed as the solution of a quadratic program (QP) \cite{Gehring13}
\begin{align}
\nonumber
\bm{F}^* =  \underset{\bm{F} \in \mathbb{R}^{12}}{\operatorname{min}}   \:\:  &(\bm{A} \bm{F} - \bm{b}_d)^T \bm{S} (\bm{A} \bm{F} - \bm{b}_d)  \\ \label{eq:BalanceControlQP} & + \alpha \| \bm{F} \|^2 + \beta \| \bm{F} - \bm{F}_{\textrm{prev}}^* \|^2\\
\mbox{s.t. }& \quad \:\:  \bm{C} \bm{F} \leq \bm{d} \nonumber
\end{align}
The cost function in \eqref{eq:BalanceControlQP} reflects a tradeoff between three goals: driving the COM dynamics to the desired values, minimizing the forces used, and penalizing deviations between the current QP solution and the solution at the previous time-step, $\bm{F}^*_{prev}$. The matrix $\bm{S}$ determines the relative priority in control over the rotational and translational motion, and the gains $\alpha > 0$ and $\beta > 0$ dictate the influence of the force normalization and solution filtering. Constraints $\bm{C} \bm{F} \leq \bm{d}$ are enforced to ensure that the optimized forces lie in the friction pyramid and that the normal forces lie within feasible bounds; these switch between support-leg and swing-leg bounds according to the scheduled contact, $\legStateScheduled$, as described in Section \ref{sec:GP}. 









==> Sections/Kinematics.tex <==
%!TEX root = ../Main.tex
\subsection{Controller Model}
Due to the irregularities of the hybrid nature arising from the repeated contact mode switches as legs enter or leave stance or swing, it is often difficult to use traditional control methods for balancing the robots. Rapidly transitioning between periods of underactuation make the problem even more complex. Therefore, the controllers used on the robot make use of a simplified control model templates to optimize ground reaction forces at the footstep locations. 


By design, the robot has light limbs with low inertia as compared to the overall body. For this reason, we can reasonably simplify the control model to ignore the effects of the legs for planning ground reaction forces from the stance feet. In particular, the Cheetah 3 controller model employs a commonly used linear relationship \cite{Focchi17,StephensAtkeson10b} between the robot's COM translational $\ddot{\pos}_{c}$ and body angular acceleration $\dot \bom_b$ and the forces $\bm{F} = (\bm{F}_1^T, \bm{F}_2^T, \bm{F}_3^T, \bm{F}_4^T)^T$ acting on each of the robot's four feet. The controller model is given by
\begin{align}
\label{eq:linear_model}
\underbrace{\left[\begin{array}{ccc} \mathbf{I}_3 & \dots & \mathbf{I}_3  \\ \hspace{-0.1cm}[\bm{p}_{1} - \pos_{c}] \times & \dots & [\bm{p}_{4} - \pos_{c}] \times \end{array} \right]}_{\bm{A}} \bm{F} = \underbrace{\left[\begin{array}{c} m (\ddot{\pos}_{c} +\bm{g}) \\ \bm{I}_G \dot \bom_b \end{array} \right]}_{\bm{b}},
\end{align}
where $m$ and $\bm{I}_G$ are the robot's total mass and centroidal rotational inertia, $\bm{g}$ is the gravity vector and $\bm{p}_{i}, i \in \{1,2,3,4\}$ are the positions of the feet. The term $[\bm{p}_{i} - \pos_{c}] \times$ is the skew-symmetric matrix representing the cross product $(\bm{p}_{i} - \pos_{c}) \times  \bm{F}_i$. 
% expressed in the notation of \cite{StephensAtkeson10b}.





==> Sections/LandingControl.tex <==
\section{Landing Controller}
\label{sec:LandingControl}
Having introduced the jumping controller, in this Section we present a force-based controller to handle impact and balance the whole body motion during the landing phase. Due to model mismatch between simulation and experiment, there is a significant pitch angle error when the robot is about to land either on the table or the ground. Therefore, the landing controller plays a crucial role to recover the robot from unexpected landing configurations. The experimental validation of this controller also proves clearly the ability to handle hard impact and control ground reaction forces of the hardware design in general and the motors in particular.

\subsection{Contact Detection}
\label{subsec:contact_detection}
Firstly, we will present the contact detection method we use to trigger the switch from the jumping controller presented in Section \ref{sec:JumpingControl} to the landing controller.

For walking experiments in the Cheetah 3 robot, we need to use a complex contact fusion algorithm based on gait timing and other criteria (see \cite{bledt2018contact}). 
For jumping behavior, because the real jumping time is normally far off from the expected value and its ground impact is much harder than that of walking, we simply detect the impact and switch to the landing control using the following condition:
\begin{align*}
&\textbf{if}~~(t\ge T_{posing}) \& (\text{any}~ \dot q_{knee,i}\ge \dot q_{knee,impact})\\
&\textbf{then}~~~\text{switch to landing control},
\end{align*}
where $T_{posing}$ is the instant when the desired trajectory is set to pose the robot in a static configuration to prepare for landing (after that time the desired knee velocity $\dot q_{knee,d}=0$); $\dot q_{knee,i}$ is the knee velocity of the $i^{th}$ foot; and $\dot q_{knee,impact}$ is the knee velocity threshold to determine if the ground impact happened.

Using this contact detection, we also clarify between three different contact models: front-leg contact; rear-leg contact; and all-leg contact. It will help the landing controller to determine which robot model should be used.

\subsection{Controller Model}
While in the trajectory optimization process, we use a detailed dynamical model of the robot described in Section \ref{sec:JumpingControl}, a simplified control model is used to optimize the ground reaction forces for balancing the whole body motion after impact, enabling a formation of real-time optimal controller.

By design, the robot has light limbs with low inertia as compared to the overall body. Therefore, it is reasonable to ignore the effects of the legs into the whole body motion for planning ground reaction forces. This assumption is also commonly used in control of legged robots \cite{Focchi17,StephensAtkeson10b}. The following linear model is then derived:
\begin{align}
\label{eq:linear_model}
\underbrace{\left[\begin{array}{ccc} \mathbf{I}_3 & \dots & \mathbf{I}_3  \\ \hspace{-0.1cm}[\bm{p}_{1} - \pos_{c}] \times & \dots & [\bm{p}_{4} - \pos_{c}] \times \end{array} \right]}_{\bm{A}} \bm{F} = \underbrace{\left[\begin{array}{c} m (\ddot{\pos}_{c} +\bm{g}) \\ \bm{I}_G \dot \bom_b \end{array} \right]}_{\bm{b}},
\end{align}
where $m$ and $\bm{I}_G$ are the robot's total mass and centroidal rotational inertia, $\bm{g}$ is the gravity vector and $\bm{p}_{i}, i \in \{1,2,3,4\}$ are the positions of the feet. The term $[\bm{p}_{i} - \pos_{c}] \times$ is the skew-symmetric matrix representing the cross product $(\bm{p}_{i} - \pos_{c}) \times  \bm{F}_i$. 
% expressed in the notation of \cite{StephensAtkeson10b}.

\subsection{Force-based Landing Controller}\label{sec:QP}
%Inspired by the controller described in \cite{Focchi17}, our landing controller enforces PD control on the center of mass and body orientation, while also ensuring that foot forces satisfy friction constraints as well as minimum and maximum ground reaction forces. The PD control law is given by 
For the landing controller, we adopted the controller described in \cite{Focchi17} with slight modification. This controller enforces PD control on the center of mass and body orientation, while also ensuring that foot forces satisfy friction constraints as well as minimum and maximum ground reaction forces. The PD control law is given by 
\begin{align}
\label{eq:pd_dynamics}
\left[\begin{array}{c}  \ddot{\pos}_{c,d} \\  \dot \bom_{b,d} \end{array} \right] = \left[\begin{array}{c}  \bm{K}_{p,p}(\pos_{c,d}-\pos_{c}) + \bm{K}_{d,p} (\dot{\pos}_{c,d}-\dot{\pos}_{c}) \\  \hspace{-0.1cm} \bm{K}_{p,\omega} \log(\bm{R}_d \bm{R}^T) +  \bm{K}_{d,\omega}(\bom_{b,d} - \bom)\end{array} \right].
\end{align}
The desired angular acceleration reflects PD control on $SO(3)$ wherein the desired and actual body orientations are described using rotation matrices $\bm{R}_d$ and $\bm{R}$, respectively, and the orientation error is obtained using the exponential map representation of rotations    \cite{Bullo95,MurrayLiSastry94}.


The goal of this controller is to resolve an optimal distribution of leg forces $\bm{F}$ that drive the approximate COM dynamics to the corresponding desired dynamics given by
\begin{align}
\bm{b}_d = \left[\begin{array}{c} m (\ddot{\pos}_{c,d} +\bm{g}) \\ \bm{I}_G \,\dot \bom_{b,d} \end{array} \right].
\end{align}
Since the model \eqref{eq:linear_model} is linear, the controller can naturally be expressed as a quadratic program (QP) \cite{Gehring13}, that can be solved in real-time of $1~kHz$: 
\begin{align}
\nonumber
\bm{F}^* =  \underset{\bm{F} \in \mathbb{R}^{12}}{\operatorname{min}}   \:\:  &(\bm{A} \bm{F} - \bm{b}_d)^T \bm{S} (\bm{A} \bm{F} - \bm{b}_d)  \\ \label{eq:BalanceControlQP} & + \alpha \| \bm{F} \|^2 + \beta \| \bm{F} - \bm{F}_{\textrm{prev}}^* \|^2\\
\mbox{s.t. }& \quad \:\:  \bm{C} \bm{F} \leq \bm{d} \nonumber\\
& \quad \:\: \bm{F}_{swing}^z=\bm{0} \nonumber
\end{align}
The cost function in \eqref{eq:BalanceControlQP} represents three goals: driving the COM to the desired dynamics, minimizing the force commands, and filtering the change of the solution $\bm{F}^*$ with respect to the previous time-step, $\bm{F}^*_{prev}$. The weight parameters $\bm{S}, \alpha, \beta$ reflect the relative priority in different elements. Constraints $\bm{C} \bm{F} \leq \bm{d}$ ensure that the optimized forces stay inside the friction pyramid and that the normal forces lie within feasible bounds.

Based on the contact model coming out from the contact detection, the normal forces of swing legs are constrained to be zeros, $\bm{F}_{swing}^z=\bm{0}$. Having this constraint in addition to the friction cone constraints in the QP controller, we will enforce the force vectors of the swing legs to be zeros, $\bm{F}_{swing}=0$. The swing legs are then kept at the posing position using PD control described in Section \ref{sec:JumpingControl} until the contact detection in those legs are triggered.

\begin{remark}
	Note that, we initially try to set all legs to be stance legs whenever we detect ground impact at any legs. However, in experiment, the robot normally has a rear-leg contact with the desk or ground first with a significant pitch angle offset at impact (see Figures \ref{fig:JumpingUp75cmBoxSnapShots} and \ref{fig:JumpingDown75cmBoxSnapShots}). Therefore, if we apply force control for all legs in this configuration, the front legs will extend fast, leading to excessive impact force and knee velocity post-impact. Switching from swing phase using position control to stance phase using force control properly helped us to overcome this issue. 
\end{remark}


==> Sections/LeastSquaresPitchPlane.tex <==
%!TEX root = ../Main.tex

\subsection{Posture Adjustment on Sloped Terrain}\label{sec:LSPP}

As mentioned, part of the Cheetah 3 controller design philosophy is to create a robust algorithm without reliance on contact sensors and vision systems. To enable Cheetah to traverse stairs and sloped terrain without vision, we use measurements of each footstep location $\bm{p}_i = (p^x_i,p^y_i,p^z_i)$ to approximate the local slope of the walking surface and adjust the robot's desired posture. In particular, the walking surface is modeled as a plane
\begin{align}
\label{eq:foot_plane}
z(x,y) = a_0 + a_1 x + a_2 y.
\end{align}
Coefficients $\bm{a} = (a_0,a_1,a_2)^T$ of \eqref{eq:foot_plane} are obtained through the solution of the least squares problem 
\begin{align}
\bm{a} &= (\bm{W}^T \bm{W})^\dagger \bm{W}^T \bm{p}^z \\
\bm{W} &= \left[ \begin{array}{ccc} \mathbf{1} & \bm{p}^x & \bm{p}^y \end{array} \right]_{4 \times 3}
\end{align}
that finds the plane that best fits the collection of measurements of the most recent contact point for each leg. Note that $\bm{p}^x$, $\bm{p}^y$ and $\bm{p}^z$ contain data for each leg, e.g. $\bm{p}^x = (p^x_1,p^x_2,p^x_3,p^x_4)$, and that $(\bm{W}^T \bm{W})^\dagger$ is the Moore-Penrose pseudoinverse of $\bm{W}^T \bm{W}$. As described in Section~\ref{sec:Results}, the estimated walking surface is used to adjust the robot's posture to accommodate uneven terrain. 


==> Sections/StateEstimation.tex <==
%!TEX root = ../Main.tex

\newcommand{\estR}{{}^0{\hskip-.1em}\hat{\bm{R}}_{ \hskip.1em  b}}
\newcommand{\estRdot}{{}^0{\hskip-.1em}\dot{\hat{\bm{R}}}_{ \hskip.1em  b}}


\subsection{State Estimation}\label{sec:State_Estimation}

Cheetah 3 estimates is it body states through a two-stage sensor fusion algorithm that decouples estimation of body orientation from estimation of the body position and velocity. It first uses its IMU to estimate orientation. Following this stage, it then fuses accelerometer measurements with leg kinematics to estimate base position and velocity via a procedure inspired by \cite{Bloesch12}. A similar two-stage scheme has also been recently applied for state-estimation in the HRP2 humanoid, as reported in \cite{Flayols17}.

The first stage of the state estimation employs an orientation filter \cite{Mahony2008tac} using both the IMU gyro and accelerometer readings. The main idea of the filter is that the gyro provides an accurate reading of the high-frequency orientation dynamics, whereas the presence of a gravity bias on the accelerometer allows it to de-drift the estimate at a comparatively lower frequency. Letting  the orientation estimate $\estR$ as the orientation of the body relative to the i.c.s., the filter updates this estimate according to
 \begin{align}
\estRdot &= \estR \left[ {}^b \boldsymbol{\omega}_b + \kappa \boldsymbol{\omega}_{corr}    \right] \times
 \end{align}
 where $\kappa > 0$ is a correction gain and $\boldsymbol{\omega}_{corr}$ is a correction angular velocity to align the accelerometer reading $\bm{a}_b$ with its gravity bias 
\[
\boldsymbol{\omega}_{corr} = \frac{\bm{a}_b}{\| \bm{a}_b \|} \times \estR^T \begin{bmatrix} 0 \\ 0 \\ 1 \end{bmatrix}
\]
% the value of \kappa=0.1 is correct
The time constant of the de-drifting from this term can be approximated by $\kappa^{-1}$. 
%In practice a selection of $\kappa=0.1$ is used, and is heuristically decreased during highly-dynamic portions of the gait where $\| \bm{a}_b\| >> g$. 
In practice $\kappa$ is heuristically decreased during highly-dynamic portions of the gait where $\| \bm{a}_b\| >> g$ with
\begin{align}
\kappa = \kappa_\text{ref} \min(1, 1 - ||\bm{a}_b - g||/g)
\end{align}
where $g$ is the acceleration of gravity and $\kappa_{\text{ref}}$ is chosen as $\kappa_\text{ref} = 0.1$. This process is effective to de-drift pitch and roll, however, error accumulation on yaw is unavoidable without fusion using exteroceptive information such as vision \cite{Fallon14}.


The second stage of the state estimation uses the orientation estimate $\estR$ along with kinematic measurements from the legs to estimate the base position and velocity. In contrast to previous state estimation techniques that posed this problem as an extended Kalman Filter \cite{Bloesch12}, the two-stage approach allows this secondary fusion to be posed as a conventional Kalman filter. This simplifies analysis and tuning of the filter and guarantees that the filter equations will never diverge in finite time. 

In continuous time, the process equations are modeled as
\begin{align}
{}^0 \dot{\bm{p}}_b & = {}^0 \bm{v}_b \\
{}^0 \dot{\bm{v}}_b &=  \estR \bm{a}_b + {}^0 \bm{a}_g + \bm{w}_{\bm{v}}\\
{}^0 \dot{\bm{p}}_i &= \bm{w}_{ \bm{p}_i } ~~\forall i = \{1,\ldots,4\}
\end{align}
where ${}^0 \bm{p}_b$ is the position of the body,  ${}^0 \bm{v}_b$ its velocity, ${}^0 \bm{a}_g = [0,~ 0,~ -g]^T$ the gravitational acceleration, and ${}^0 \bm{p}_i$ the position of foot $i$. The white noise terms $\bm{w}_{\bm{v}}$ and $\bm{w}_{ \bm{p}_i }$ characterize the noise in the accelerometer and any variability in the foot positions. As in \cite{Bloesch12} the variability in the foot position is modeled to account for effects of foot slip in stance, or can also capture foot swing by inflating the process noise on that foot to a high level. Viewing $\estR \bm{a}_b + {}^0 \bm{a}_g$ as an input to the system, these equations represent a linear time invariant process, and thus are amenable to conventional Kalman filtering. The continuous time model is converted into discrete time with a 1ms time step using an identical procedure to \cite{Bloesch12}.

Leg kinematics provide measurements of the relative position vector between each foot and the body to de-drift estimates ${}^0 \hat{\bm{p}}_b$, ${}^0 \hat{\bm{v}}_b$, and ${}^0\hat{\bm{p}}_i$ for each foot. Letting ${}^0\bm{p}_{rel}(\bm{q}_i,\estR)$ denote the relative foot position as computed by kinematics, a measurement residual is generated 
\[
\bm{e}_{p,i} = \left({}^0\hat{\bm{p}}_i - {}^0 \hat{\bm{p}}_b\right) -  {}^0\bm{p}_{rel}(\bm{q}_i, \estR)
\] 
Similarly, the velocity of the foot relative to the body can be computed from the leg angles, velocities, and the body orientation and angular velocity. This computation is denoted as ${}^0\bm{p}_{rel}(\bm{q}_i,\dot{\bm{q}}_i, \estR, {}^b \boldsymbol{\omega}_b)$. Under the assumption that each foot is fixed, this provides an associated measurement residual
 \[
\bm{e}_{v,i} = \left( -{}^0 \hat{\bm{v}}_b \right) - {}^0\bm{p}_{rel}(\bm{q}_i,\dot{\bm{q}}_i, \estR, {}^b \boldsymbol{\omega}_b) 
\] 
Finally, a contact height $h_i$ is assumed for each foot  with associated measurement residual:
\[
\bm{e}_{h_i} = \left( [0,~ 0,~ 1]^T\, {}^0 \hat{{\bm{p}}}_i \right) - h_i
\]
Random multivariate Gaussian's are used to capture the measurements errors for each residual. Similar to the process noise $\bm{w}_{ \bm{p}_i }$ on the feet, measurement covariances for foot $i$ are increased to a high value during swing such that the swing leg measurements are effectively ignored in this fusion process. Although space permits a full development, the residuals are used within the innovations step of a Kalman filter to provide estimates ${}^0 \hat{\bm{p}}_b$, ${}^0 \hat{\bm{v}}_b$, and ${}^0 \hat{\bm{p}}_i$ used for feedback to the Balance Control or MPC components.



%\begin{itemize}
%\item Kalman filtering equations and virtual measurements
%\item Comments on the how the staging reduces what would other be an EKF into a KF
%\item 
%
%\end{itemize}

==> Utils/TestCommands.tex <==
% File used to test the custom commands for various equations and variables used in the paper.

% Titles the section 
\section{Test Commands}

State Variable Definitions\\
$\roll \pitch \yaw \dRoll \dPitch \dYaw \omegaX \omegaY \omegaZ\\
\quatVector \posVector \angVelVector \velVector \rpyVector \rpyDotVector\\
\stateVector \stateVectorRed \inputVector\\
\rpyVector = \quatToRPY\\
\rpyDotVector = \omegaToRPYDot\angVelVector$\\\\

Simplified Dynamics\\
$\inputForceTorqueFunction = \inputForceTorque = \forceTorqueTransform\uToForceTorqueMat\BMat{\forceEstimate_1 \\ \vdots \\ \forceEstimate_s}\\
\simpleDynamics$\\\\

Direct Collocation Decision Variables\\
$\decisionArrayVector\\
\decisionArrayVectorFull$\\\\

Model Predictive Control Formulation\\
$\basicCostFunction\\
\basicCost = \MPCCostFull\\
\stateError = \stateErrorFull\\
\inputError = \inputErrorFull\\
\basicCostFunction = \MPCCostFunction$\\

% MPC Formulation (descriptive titles)
\begin{equation*}
	\begin{matrix}
		&\MPCMin
		&   & \MPCSum\pMat{\MPCCost}_{n,k} \\\\
		& \text{subject to}
		&	& \text{Dynamics} \\
		  &   &   & \dynamicsConstraint                \\\\
		  &   &   & \text{Foot placed on ground}       \\
		  &   &   & \groundConstraint                  \\\\
		  &   &   & \text{Kinematic leg limits}        \\
		  &   &   & \kinematicLegConstraint            \\\\
		  &   &   & \text{Foot stationary in stance}   \\
		  &   &   & \slipConstraint                    \\\\
		  &   &   & \text{Lateral force friction cone} \\
		  &   &   & \frictionConstraint{x}             \\
		  &   &   & \frictionConstraint{y}             
	\end{matrix}
\end{equation*}

% MPC Formulation (just equations)
\begin{equation*}
	\begin{matrix}
		&\MPCMin
		&   & \MPCSum\pMat{\MPCCost}_{n,k} \\\\
		& \text{subject to}
		&   & \dynamicsConstraint     \\
		  &   &   & \groundConstraint       \\
		  &   &   & \kinematicLegConstraint \\
		  &   &   & \slipConstraint         \\
		  &   &   & \frictionConstraint{x}  \\
		  &   &   & \frictionConstraint{y}  \\
	\end{matrix}
\end{equation*}
